Multi-Sensor Diffusion-Driven Optical Image Translation for Large-Scale Applications

Comparing images captured by disparate sensors is a common challenge in remote sensing. This requires image translation -- converting imagery from one sensor domain to another while preserving the original content. Denoising Diffusion Implicit Models (DDIM) are potential state-of-the-art solutions for such domain translation due to their proven superiority in multiple image-to-image translation tasks in computer vision. However, these models struggle with reproducing radiometric features of large-scale multi-patch imagery, resulting in inconsistencies across the full image. This renders downstream tasks like Heterogeneous Change Detection impractical. To overcome these limitations, we propose a method that leverages denoising diffusion for effective multi-sensor optical image translation over large areas. Our approach super-resolves large-scale low spatial resolution images into high-resolution equivalents from disparate optical sensors, ensuring uniformity across hundreds of patches. Our contributions lie in new forward and reverse diffusion processes that address the challenges of large-scale image translation. Extensive experiments using paired Sentinel-II (10m) and Planet Dove (3m) images demonstrate that our approach provides precise domain adaptation, preserving image content while improving radiometric accuracy and feature representation. A thorough image quality assessment and comparisons with the standard DDIM framework and five other leading methods are presented. We reach a mean Learned Perceptual Image Patch Similarity (mLPIPS) of 0.1884 and a Fr\'echet Inception Distance (FID) of 45.64, expressively outperforming all compared methods, including DDIM, ShuffleMixer, and SwinIR. The usefulness of our approach is further demonstrated in two Heterogeneous Change Detection tasks.

==> tikz/inference_diag.tex <==
\tikzset{every picture/.style={line width=0.75pt}} 
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,340); %set diagram left start at 0, and has height of 340

%Image [id:dp5165325364706224] 
\draw (135.7,90.7) node  {\includegraphics[width=44.55pt,height=44.55pt]{figs/globalinput_11-58-28.jpg}};
%Shape: Rectangle [id:dp38344809167160876] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]  (106,61) -- (165.39,61) -- (165.39,120.39) -- (106,120.39) -- cycle ;
%Image [id:dp4648246210324154] 
\draw (135.7,167.06) node  {\includegraphics[width=44.55pt,height=44.55pt]{figs/localinput_14-03-38.jpg}};
%Shape: Rectangle [id:dp44056947170380445] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]  (106,137.36) -- (165.39,137.36) -- (165.39,196.76) -- (106,196.76) -- cycle ;

%Straight Lines [id:da10658113710102013] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (165.39,91) -- (203.58,91) ;
%Straight Lines [id:da044949075276068395] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (203.58,91) -- (203.58,110.21) ;
\draw [shift={(203.58,112.21)}, rotate = 270] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;

%Straight Lines [id:da6706122128002383] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (165.39,167.36) -- (203.58,167.36) ;
%Straight Lines [id:da1786942867270167] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (203.58,167.36) -- (203.58,148.15) ;
\draw [shift={(203.58,146.15)}, rotate = 90] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;

%Straight Lines [id:da725835811412701] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (233.27,128.88) -- (252.48,128.88) ;
\draw [shift={(254.48,128.88)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Shape: Rectangle [id:dp435589503238057] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]  (330,116) -- (380.91,116) -- (380.91,141.64) -- (330,141.64) -- cycle ;

%Straight Lines [id:da00002105785629802348] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (308.88,128.88) -- (328.09,128.88) ;
\draw [shift={(330.09,128.88)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Straight Lines [id:da911954216614036] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (381.5,128.88) -- (393.82,128.88) -- (403.5,128.88) ;
\draw [shift={(405.5,128.88)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Shape: Rectangle [id:dp16454750961647768] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]  (382.37,214) -- (463.28,214) -- (463.28,249) -- (382.37,249) -- cycle ;

%Straight Lines [id:da03748232226700088] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (479.28,232) -- (465.28,232) ;
\draw [shift={(463.28,232)}, rotate = 360] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Straight Lines [id:da6342060529065483] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (502.8,148) -- (502.8,161) ;
\draw [shift={(502.8,163)}, rotate = 270] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;

%Shape: Rectangle [id:dp48786368230164556] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]  (464,113) -- (544.91,113) -- (544.91,148) -- (464,148) -- cycle ;
%Image [id:dp19663652035411427] 
\draw (503.09,232.29) node  {\includegraphics[width=35.56pt,height=35.56pt]{figs/noise_12-31-35.jpg}};
%Shape: Rectangle [id:dp48297649621798455] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]  (479.38,208.58) -- (526.8,208.58) -- (526.8,256) -- (479.38,256) -- cycle ;

%Straight Lines [id:da7532077525852792] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (502.8,193) -- (502.8,206) ;
\draw [shift={(502.8,208)}, rotate = 270] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Straight Lines [id:da426561530558325] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (444,130) -- (462,130) ;
\draw [shift={(464,130)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Straight Lines [id:da6243702138562277] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (422,144) -- (422,178) ;
%Straight Lines [id:da5373479552691811] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (422,178) -- (478,178) ;
\draw [shift={(480,178)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;

%Shape: Parallelogram [id:dp8510124238919192] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]  (410.12,116) -- (446.78,116) -- (438.26,142.83) -- (401.59,142.83) -- cycle ;
%Straight Lines [id:da1326826065941924] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (502.8,97) -- (502.8,110) ;
\draw [shift={(502.8,112)}, rotate = 270] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Image [id:dp08909454703748554] 
\draw (494.51,61.71) node  {\includegraphics[width=35.56pt,height=35.56pt]{figs/noise_12-31-35.jpg}};
%Shape: Rectangle [id:dp14762183216666624] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]  (470.8,38) -- (518.22,38) -- (518.22,85.42) -- (470.8,85.42) -- cycle ;

%Image [id:dp6465516646053848] 
\draw (498.5,65.7) node  {\includegraphics[width=35.56pt,height=35.56pt]{figs/noise_12-31-35.jpg}};
%Shape: Rectangle [id:dp04938416779796406] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]  (474.79,41.99) -- (522.21,41.99) -- (522.21,89.41) -- (474.79,89.41) -- cycle ;

%Image [id:dp03133041776454504] 
\draw (502.49,69.69) node  {\includegraphics[width=35.56pt,height=35.56pt]{figs/noise_12-31-35.jpg}};
%Shape: Rectangle [id:dp8918408011877201] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]  (478.78,45.98) -- (526.2,45.98) -- (526.2,93.4) -- (478.78,93.4) -- cycle ;

%Image [id:dp7229165049230586] 
\draw (506.48,73.68) node  {\includegraphics[width=35.56pt,height=35.56pt]{figs/noise_12-31-35.jpg}};
%Shape: Rectangle [id:dp8272589957071823] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]  (482.77,49.98) -- (530.19,49.98) -- (530.19,97.39) -- (482.77,97.39) -- cycle ;


%Shape: Rectangle [id:dp5424860062923536] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]  (480.59,164.14) -- (525.59,164.14) -- (525.59,193.08) -- (480.59,193.08) -- cycle ;

%Shape: Rectangle [id:dp7374159529934188] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]  (174.61,111.91) -- (233.27,111.91) -- (233.27,145.85) -- (174.61,145.85) -- cycle ;

%Straight Lines [id:da41230722743045134] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (382.39,232.61) -- (368.39,232.61) ;
\draw [shift={(366.39,232.61)}, rotate = 360] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Shape: Parallelogram [id:dp5448478966246932] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]  (331.9,180) -- (360,180) -- (354.1,202) -- (326,202) -- cycle ;

%Straight Lines [id:da21514957754494946] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (342.39,202.88) -- (342.39,210.61) -- (342.39,216.88) ;
\draw [shift={(342.39,218.88)}, rotate = 270] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Image [id:dp012983772985253772] 
\draw (282.37,125.37) node  {\includegraphics[width=41.06pt,height=41.06pt]{figs/globalinput_11-58-28.jpg}};
%Shape: Rectangle [id:dp991698907384708] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]  (255,98) -- (309.74,98) -- (309.74,152.74) -- (255,152.74) -- cycle ;

%Image [id:dp3985846446540888] 
\draw (285.63,129.23) node  {\includegraphics[width=41.06pt,height=41.06pt]{figs/localinput_14-03-38.jpg}};
%Shape: Rectangle [id:dp5304412516487229] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]  (258.26,101.86) -- (313,101.86) -- (313,156.61) -- (258.26,156.61) -- cycle ;


%Image [id:dp12013835099221071] 
\draw (274.3,232.3) node  {\includegraphics[width=44.55pt,height=44.55pt]{figs/localoutput_15-42-12.jpg}};
%Shape: Rectangle [id:dp7218640132033931] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]  (244.61,202.61) -- (304,202.61) -- (304,262) -- (244.61,262) -- cycle ;

%Shape: Rectangle [id:dp06899067937676517] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]  (320.39,218.97) -- (365.3,218.97) -- (365.3,244.61) -- (320.39,244.61) -- cycle ;

%Straight Lines [id:da6181413780772338] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (319.5,232.56) -- (305.5,232.56) ;
\draw [shift={(303.5,232.56)}, rotate = 360] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;

% Text Node
\draw (175.5,115.9) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{40.39pt}\setlength\topsep{0pt}
\begin{center}
{Channel-wise \\ Stacking}
\end{center}

\end{minipage}};
% Text Node
\draw (467.8,116.59) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{52.2pt}\setlength\topsep{0pt}
\begin{center}
Reverse Diffusion\\
$N/i$ Iterations
\end{center}

\end{minipage}};
% Text Node
\draw (487.75,166.11) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{21.54pt}\setlength\topsep{0pt}
\begin{center}
pSNR\\Voting
\end{center}

\end{minipage}};
% Text Node
\draw (386.37,218.96) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {\begin{minipage}[lt]{52.2pt}\setlength\topsep{0pt}
\begin{center}
Reverse Diffusion\\
$N$ Iterations
\end{center}

\end{minipage}};

% Text Node
\draw (333,122.4) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{32.56pt}\setlength\topsep{0pt}
\begin{center}
Whitening
\end{center}

\end{minipage}};
% Text Node
\draw (324.3,225.01) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{26.98pt}\setlength\topsep{0pt}
\begin{center}
Coloring
\end{center}

\end{minipage}};
% Text Node
\draw (123,43.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\mathbf{I}_{\text{in}}^{\text{LR,global}}$};
% Text Node
\draw (123,199.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\mathbf{I}_{\text{in}}^{\text{LR,local}}$};
% Text Node
\draw (274,80.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\mathbf{I}_{\text{in}}^{\text{LR}}$};
% Text Node
\draw (416,120.4) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$\mathbf{X}$};
% Text Node
\draw (263,264.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\mathbf{I}_{\text{out}}^{\text{HR,local}}$};
% Text Node
\draw (493,257.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\mathbf{\epsilon }_{T}^{\text{best}}$};
% Text Node
\draw (487,19.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\mathbf{\epsilon}_{T}^{\text{best}}$};
% Text Node
\draw (333.9,183.4) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$\mathbf{c}_{\text{out}}$};


\end{tikzpicture}


==> tikz/training_diag.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,229); %set diagram left start at 0, and has height of 229

%Shape: Rectangle [id:dp1331758405300827] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]  (373.24,25.36) -- (322.33,25.36) -- (322.33,51) -- (373.24,51) -- cycle ;
%Straight Lines [id:da8493319704290669] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (395.55,37.36) -- (376.33,37.36) ;
\draw [shift={(374.33,37.36)}, rotate = 360] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Straight Lines [id:da6390412267689314] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (321.55,37.36) -- (302.33,37.36) ;
\draw [shift={(300.33,37.36)}, rotate = 360] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;

%Shape: Rectangle [id:dp006486740837236882] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]  (90.33,23.39) -- (141.24,23.39) -- (141.24,49.03) -- (90.33,49.03) -- cycle ;

%Straight Lines [id:da9352751190388904] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (68.33,35.39) -- (87.55,35.39) ;
\draw [shift={(89.55,35.39)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Image [id:dp13773371291480707] 
\draw (38.03,34.7) node  {\includegraphics[width=44.55pt,height=44.55pt]{figs/localoutput_15-42-12.jpg}};
%Shape: Rectangle [id:dp8230478368846841] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]  (8.33,5) -- (67.73,5) -- (67.73,64.39) -- (8.33,64.39) -- cycle ;


%Straight Lines [id:da1406400718913572] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (142.33,35.39) -- (161.55,35.39) ;
\draw [shift={(163.55,35.39)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Straight Lines [id:da5051188779647056] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (176.33,113.39) -- (176.33,99.39) ;
\draw [shift={(176.33,97.39)}, rotate = 90] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Straight Lines [id:da34306351374183364] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (132.33,85.39) -- (149.55,85.39) ;
\draw [shift={(151.55,85.39)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Shape: Parallelogram [id:dp3769612192376086] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]  (113.04,73) -- (134.33,73) -- (130.11,97) -- (108.82,97) -- cycle ;

%Straight Lines [id:da8504283334521427] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (176.33,47.39) -- (176.33,65.39) ;
\draw [shift={(176.33,67.39)}, rotate = 270] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Shape: Parallelogram [id:dp9971136997616132] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]  (166.37,23.39) -- (194.33,23.39) -- (188.78,47.39) -- (160.82,47.39) -- cycle ;

%Image [id:dp05688128377717527] 
\draw (421.71,32.37) node  {\includegraphics[width=41.06pt,height=41.06pt]{figs/globalinput_11-58-28.jpg}};
%Shape: Rectangle [id:dp12769414685458536] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]  (394.33,5) -- (449.08,5) -- (449.08,59.74) -- (394.33,59.74) -- cycle ;

%Image [id:dp9886869861737808] 
\draw (424.96,36.23) node  {\includegraphics[width=41.06pt,height=41.06pt]{figs/localinput_14-03-38.jpg}};
%Shape: Rectangle [id:dp3507610516243711] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]  (397.59,8.86) -- (452.33,8.86) -- (452.33,63.61) -- (397.59,63.61) -- cycle ;


%Straight Lines [id:da6183841318378611] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (284.33,47) -- (284.33,65.58) ;
\draw [shift={(284.33,67.58)}, rotate = 270] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Shape: Parallelogram [id:dp22054158651099298] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]  (272.47,23.79) -- (304.73,23.79) -- (297.23,47.39) -- (264.97,47.39) -- cycle ;

%Shape: Parallelogram [id:dp6091463580095875] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]  (223.38,72.39) -- (246.33,72.39) -- (241.78,96.15) -- (218.82,96.15) -- cycle ;

%Straight Lines [id:da25082888632425315] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (201.12,85.39) -- (218.33,85.39) ;
\draw [shift={(220.33,85.39)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Straight Lines [id:da02091919632250616] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (244.12,85.39) -- (261.33,85.39) ;
\draw [shift={(263.33,85.39)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Image [id:dp32777376954631143] 
\draw (285.29,137.1) node  {\includegraphics[width=35.56pt,height=35.56pt]{figs/noise_12-31-35.jpg}};
%Shape: Rectangle [id:dp7957921485946566] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]  (261.58,113.39) -- (309,113.39) -- (309,160.81) -- (261.58,160.81) -- cycle ;

%Straight Lines [id:da5887505649518194] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (284.33,98.58) -- (284.33,110.58) ;
\draw [shift={(284.33,112.58)}, rotate = 270] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;
%Shape: Rectangle [id:dp446689002739193] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]  (264.33,68) -- (306.33,68) -- (306.33,97) -- (264.33,97) -- cycle ;
%Image [id:dp7160172697705682] 
\draw (176.62,137.1) node  {\includegraphics[width=35.56pt,height=35.56pt]{figs/noise_12-31-35.jpg}};
%Shape: Rectangle [id:dp5872634943645958] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=0.75]  (152.91,113.39) -- (200.33,113.39) -- (200.33,160.81) -- (152.91,160.81) -- cycle ;

%Shape: Rectangle [id:dp40227331057405835] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]  (206.33,169.5) -- (256.33,169.5) -- (256.33,193.5) -- (206.33,193.5) -- cycle ;
%Shape: Rectangle [id:dp7022418059082376] 
\draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]  (152.33,68.39) -- (200.33,68.39) -- (200.33,97.39) -- (152.33,97.39) -- cycle ;

%Straight Lines [id:da35397078573477603] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (200.66,137) -- (226.33,137) ;
%Straight Lines [id:da5262160824613367] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (226.33,137) -- (226.33,167) ;
\draw [shift={(226.33,169)}, rotate = 270] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;

%Straight Lines [id:da6189929755908787] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (238.33,137) -- (261.55,137) ;
%Straight Lines [id:da08958559486867856] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ]   (238.33,137) -- (238.33,167) ;
\draw [shift={(238.33,169)}, rotate = 270] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (7.2,-1.8) -- (0,0) -- (7.2,1.8) -- cycle    ;


% Text Node
\draw (93.33,29.79) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{32.56pt}\setlength\topsep{0pt}
\begin{center}
Whitening
\end{center}

\end{minipage}};
% Text Node
\draw (26.73,66.79) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\mathbf{I}_{\text{out}}^{\text{HR,local}}$};
% Text Node
\draw (170.82,27.79) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$\mathbf{y}_{0}$};
% Text Node
\draw (114.88,77.4) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$\gamma _{t}$};
% Text Node
\draw (276.63,26.63) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$\mathbf{X}$};
% Text Node
\draw (157.33,70.79) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{28.18pt}\setlength\topsep{0pt}
\begin{center}
Forward\\Diffusion
\end{center}

\end{minipage}};
% Text Node
\draw (226.08,75.79) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$\tilde{\mathbf{y}}_{t}$};
% Text Node
\draw (171.33,161.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\mathbf{\epsilon }$};
% Text Node
\draw (281.33,166.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\hat{\mathbf{\epsilon }}$};
% Text Node
\draw (267.33,70.4) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{26.62pt}\setlength\topsep{0pt}
\begin{center}
Neural\\Network
\end{center}

\end{minipage}};
% Text Node
\draw (325.33,32.4) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{32.56pt}\setlength\topsep{0pt}
\begin{center}
Whitening
\end{center}

\end{minipage}};
% Text Node
\draw (419.33,66.79) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\mathbf{I}_{\text{in}}^{\text{LR}}$};
% Text Node
\draw (211.58,172.4) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$\mathcal{L}(\mathbf{\epsilon } ,\boldsymbol{\hat{\mathbf{\epsilon }}})$};


\end{tikzpicture}

